Exploring Robustness of Multilingual LLMs on Real-World Noisy Data

Large Language Models (LLMs) are trained on Web data that might contain spelling errors made by humans. But do they become robust to similar real-world noise? In this paper, we investigate the effect of real-world spelling mistakes on the performance of 9 language models, with parameters ranging from 0.2B to 13B, in 3 different NLP tasks, namely Natural Language Inference (NLI), Name Entity Recognition (NER), and Intent Classification (IC). We perform our experiments on 6 different languages and build a dictionary of real-world noise for them using the Wikipedia edit history. We show that the performance gap of the studied models on the clean and noisy test data averaged across all the datasets and languages ranges from 2.3 to 4.3 absolute percentage points. In addition, mT5 models, in general, show more robustness compared to BLOOM, Falcon, and BERT-like models. In particular, mT5 (13B), was the most robust on average overall, across the 3 tasks, and in 4 of the 6 languages.

==> images/average_of_all.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar stacked,
    ymin=0,
    xtick=data,
    xticklabels={mBERT-179M, XLM-R-279M, mT5-300M, mT5-580M, mT5-1B, mT5-3B, BLOOM-7B, Falcon-7B, mT5-13B},
    ylabel={Performance Gap},
    y label style={at={(axis description cs:+0.07,.5)}, font=\tiny},
    xlabel={},
    y tick label style={font=\tiny},
    width=0.5\textwidth,
    height=6.6cm,
    ymax=17,
    bar width=0.47cm,
    legend style={at={(0.5,0.98)},
      anchor=north,legend columns=-1,font=\tiny},
    x tick label style={rotate=45, anchor=east, font=\tiny},
    ymajorgrids=true,
    grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50}
    ]
    
\addplot [fill=blue!15, postaction={pattern=crosshatch}] coordinates {
    (1, 6.47)
    (2, 6.12)
    (3, 4.48)
    (4, 5.87)
    (5, 5.48)
    (6, 5.14)
    (7, 5.38)
    (8, 5.70)
    (9, 4.37)
};

\addplot [fill=red!20, postaction={pattern=dots}] coordinates {
    (1, 3.87)
    (2, 3.43)
    (3, 2.01)
    (4, 2.16)
    (5, 2.06)
    (6, 2.57)
    (7, 8.32)
    (8, 4.69)
    (9, 1.94)
};

\addplot [fill=green!20, postaction={pattern=crosshatch dots}] coordinates {
    (1, 0.72)
    (2, 0.54)
    (3, 0.94)
    (4, 0.65)
    (5, 0.52)
    (6, 0.27)
    (7, 0.59)
    (8, 0.62)
    (9, 0.34)
};

\legend{XLNI (NLI), Wikiann (NER), SNIPS (IC)}
\end{axis}
\end{tikzpicture}
\caption{Average performance gap (in percentage points) between the model accuracy on the clean and noisy data across 6 languages aggregated over the datasets for the models in our study.}
\label{fig:c-n-average_of_all}

\end{figure}

==> tables/dataset_wrong_ex.tex <==

% \begin{table*}[t]

%     \centering
%     \small
%     % \ttfamily
%     % \renewcommand{\arraystretch}{2}
%     \setlength{\tabcolsep}{3pt}
%     \begin{tabularx}{\linewidth}{c c X c c}
%         \hline
%          \textbf{Language} & \textbf{Source} &  \multicolumn{1}{c}{\textbf{Text}} & \textbf{Predicted Label} & \textbf{True Label} \\[1pt]
%          \hline
         
%          % \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{XNLI}}}
%         \multicolumn{5}{c}{\textbf{XNLI}} \\
%         \hline
%          \multirow{2}{*}{English} 
%          & clean & Why did you let Wolverstone and the others go?  he cried, with a touch of bitterness., Wolverstone was not the only person who left. &1 &0\\
%          & noisy & Why ded you set Wolverstone and the others go? he cried , with a touch of bitterness., Wolverstone las not the only person who deft. & 1& 0\\[5pt] 
        
%           \multirow{2}{*}{German} 
%          & clean & Warum haben Sie Wolverstone und die anderen gehen lassen?, rief er mit ein bisschen Groll in der Stimme.', 'Wolverstone war nicht die einzige Person, die ging. & 1 &0\\
%          & noisy & Warum haben Sie Wolverstone und die anderen gehen lassen? , rief er mit ein bissschen Groll in eder Stimme ., Wolverstone warr nicht wie einzige Person , die ging. & 1&0\\[5pt] 

%          \multirow{2}{*}{Spanish} 
%          & clean& Por qué dejaste ir a Wolverstone y a los demás? Gritó con un toque de amargura., Wolverstone no fue la única persona que se fue.& 1 &0\\
%          & noisy & Por que dejaste ir a Wolverstone y a los demás? Gritó con un toque ae atargura., Wolverstone no fue la única persona que se fuee. &1&0\\[5pt] 

%         \multirow{2}{*}{French} 
%          & clean & Pourquoi avez-vous laissé Wolverstone et les autres partir ? cria-t-il, avec une touche d'amertume., Wolverstone n'est pas la seule personne a être partie.& 1&0 \\
%          & noisy & Pourquoi avez-vous laissé Wolverstone et les autre partir ? cria-t-il , avec una touche d'amertume ., Wolverstone n'est pas la yeule personne a être parctie.& 2&0\\[5pt] 
%         \multirow{2}{*}{Hindi} 
%          & clean &  {\hindifont आप ने वूल्वरस्टोन और अन्य लोगों को क्यों जाने दिया? वह दुःख महसूस करने के साथ रो दिया|, वूल्वरस्टोन अकेला व्यक्ति नहीं था जो चला गया।} &2&0\\
%          & noisy &  {\hindifont यह ने वूल्वरस्टोन और अन्य लोगों को क्यों जाने दिया? मई दुःख महसूस करने के साथ रो दिया|, वूल्वरस्टोन अकेला व्यक्ति नहीं था जो एका गया।}& 2&0\\[5pt] 

%         \multirow{2}{*}{Turkish} 
%          & clean & Acıklı bir dokunuşla haykırdı; Wolverstone'un ve diğerlerinin gitmesine neden izin verdin?, Wolverstone giden tek insan değildi.& 1&0\\
%          & noisy & Acıklı birr dokunuşla haykırdı; Wolverstone'un ve dikğerlerinin gitmesine neden izin verdin?, Wolverstone giden telk insan değildi.& 2&0\\[2pt] 
         
%         \hline
%         \multicolumn{5}{c}{\textbf{SNIPS}} \\
%         \hline
%          \multirow{2}{*}{English} 
%          & clean & I want to hear the album Suites \& Sweets.&3&3\\
%          & noisy & I want to thear the album Suites \& Sweets.&5&3\\[5pt] 
        
%           \multirow{2}{*}{German} 
%          & clean & Ich will das Album Suites \& Sweets hören.&3&3\\
%          & noisy & Ich will das Album Suites \& Sweets hörten.&5&3\\[5pt] 

%          \multirow{2}{*}{Spanish} 
%          & clean&Quiero escuchar el álbum Suites \& Sweets.&3&3\\
%          & noisy & Quiero excuchar el álbum Suites \& Sweets.&5&3\\[5pt] 

%         \multirow{2}{*}{French} 
%          & clean & Je veux écouter l'album Suites \& Sweets.&3&3\\
%          & noisy & Je veut écouter l'album Suites \& Sweets.&5&3\\[5pt] 
         
%        \multirow{2}{*}{Hindi} 
%          & clean &  {\hindifont मैं एल्बम सुइट्स और मिठाई सुनना चाहते हैं।}&3&3\\
%          & noisy & {\hindifont मैं एल्बम सुइट्स रख मिठाई सुनना चाहते हैं।}&5&3\\[5pt] 

%         \multirow{2}{*}{Turkish} 
%          & clean & Suites \& Sweets albümünü dinlemek istiyorum.&3&3\\
%          & noisy & Suites \& Sweets albümünü dinlemek ittiyorum.&5&3\\[2pt] 

%          \hline

%         \multicolumn{5}{c}{\textbf{WikiANN}} \\
%         \hline
%          \multirow{2}{*}{English} 
%          & clean & : On Lifetime Channel &[O, O, B-ORG, I-ORG]
% \\
%          & noisy & : On Liferime Channel& [O, O, O, I-ORG]
% \\[5pt] 
        
%           \multirow{2}{*}{German} 
%          & clean &  " Michigan " & [O, O, O, O, O] \\
%          & noisy & " Michigyn "& [O, O, B-PER, O, O]\\[5pt] 

%          \multirow{2}{*}{Spanish} 
%          & clean&REDIRECCIÓN Comité Olímpico Brasileño &[O, B-ORG, I-ORG, I-ORG]\\
%          & noisy & REDIRECCIÓN Comité Olímpico Braslleño & [O, O, I-ORG, I-ORG]\\[5pt] 

%         \multirow{2}{*}{French} 
%          & clean & 'Potentilla erecta' &[O, B-LOC, I-LOC, O]\\
%          & noisy & 'Potentilla erecga' &[O, O, I-LOC, O]\\[5pt] 


%         \multirow{2}{*}{Turkish} 
%          & clean & Tang Hanedanı kuruldu.
%          & [B-LOC, I-LOC, O, O]\\
%          & noisy & Tang Hanecanı kuruldu.
%          & [B-ORG, I-LOC, O, O]\\[2pt] 

%          \hline
         
%     \end{tabularx}
    
%     \caption{Clean and noisy tests that are classified wrongly in all models.}
%     \label{tab:Noisy_wrong_predicted}
    
% \end{table*}

==> tables/noisy_test_examples.tex <==

\begin{table*}[t]

    \centering
    \small
    % \ttfamily
    % \renewcommand{\arraystretch}{2}
    \setlength{\tabcolsep}{10pt}
    \begin{tabularx}{\linewidth}{c c X }
        \hline
         & \textbf{Language} &  \multicolumn{1}{c}{\textbf{Noisy Test}}   \\[1pt]
         \hline
         \\
         \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{SNIPS}}}
        
        & English  & Please \textcolor{red}{suarch} \textcolor{red}{por} the television show , Episodi di The Blacklist.\\[5pt] 
        
       & German & Wo ist das nächstgelegene Kino , das \textcolor{red}{alsländische} Filme zeigte? \\[5pt]
        
        &Spanish & Puedes \textcolor{red}{incontrarme} el remolque de Blue Spring?\\[5pt]
        
        &French & Dites-moi la météo \textcolor{red}{jour} 6h dans le \textcolor{red}{partc} national des Tatras. \\[5pt]
     
         & Hindi & {\hindifont कृपया उपर देखो \textcolor{red}{नए} मुझे हॉलीवुड बाउल में मोंटी पायथन लाइव ढूंढो} \\[5pt]
        
        &Turkish & Nebraska \textcolor{red}{üçin} hava tahminini kontrol et. \\[5pt]
        \hline
         
         \\
         
         \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{XNLI}}}
        
        & English  & \textcolor{red}{Wednesday}, Clinton chose \textcolor{red}{lo} talk about a \textcolor{red}{defferent} industry.\\[5pt] 
        
       & German & Wir versperren \textcolor{red}{onseren} \textcolor{red}{einetritt} in die technologische \textcolor{red}{zumkunft}. \\[5pt]
        
        &Spanish & La Figura 4 muestra la curva de \textcolor{red}{oherta} de los \textcolor{red}{lervicios} de \textcolor{red}{trabajó} compartido.\\[5pt]
        
        &French & Ajaj est entré aux États-Unis avec \textcolor{red}{une} visa touristique B-2 à New-York \textcolor{red}{se} 9 \textcolor{red}{svptembre} 1991. \\[5pt]
     
         & Hindi & {\hindifont \textcolor{red}{वहें} अस्पे खर्च \textcolor{red}{मईे} जिसके पास मौका हो।} \\[5pt]
        
        &Turkish & Balkinger’\textcolor{red}{en} uyarıları \textcolor{red}{üçin} Ed Ballinger’in röportajına bakınız (14 \textcolor{red}{zisan} 2004). \\[5pt]
        \hline\\[1pt]
        \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Wikiann}}}
         & English &  Unicoi County, \textcolor{red}{Tennesxee}.\\[5pt]
         & German &  Er unterschrieb \textcolor{red}{brim} zweitklassigen Gazélec FC Ajaccio auf Korsika.\\[5pt]
         & Spanish &  REDIRECCIÓN Sebastián \textcolor{red}{Mirajda} Córdova.\\[5pt]
         & French & Elle traverse tout le 6 \textcolor{red}{arronxissement} d'est en ouest. \\[5pt]
         & Turkish & Izlanda - Ásgeir \textcolor{red}{Sigurvihsson}. \\[5pt]
         \hline
         
    \end{tabularx}
    
    \caption{Noisy test set samples for XNLI dataset created by WikiTypo method and the Wikiann dataset using NLPAUG library}
    \label{tab:Noisy_tests_examples}
    
\end{table*}
